Distilling Optimal Neural Networks: Rapid Search in Diverse Spaces

Current state-of-the-art Neural Architecture Search (NAS) methods neither efficiently scale to multiple hardware platforms, nor handle diverse architectural search-spaces. To remedy this, we present DONNA (Distilling Optimal Neural Network Architectures), a novel pipeline for rapid, scalable and diverse NAS, that scales to many user scenarios. DONNA consists of three phases. First, an accuracy predictor is built using blockwise knowledge distillation from a reference model. This predictor enables searching across diverse networks with varying macro-architectural parameters such as layer types and attention mechanisms, as well as across micro-architectural parameters such as block repeats and expansion rates. Second, a rapid evolutionary search finds a set of pareto-optimal architectures for any scenario using the accuracy predictor and on-device measurements. Third, optimal models are quickly finetuned to training-from-scratch accuracy. DONNA is up to 100x faster than MNasNet in finding state-of-the-art architectures on-device. Classifying ImageNet, DONNA architectures are 20% faster than EfficientNet-B0 and MobileNetV2 on a Nvidia V100 GPU and 10% faster with 0.5% higher accuracy than MobileNetV2-1.4x on a Samsung S20 smartphone. In addition to NAS, DONNA is used for search-space extension and exploration, as well as hardware-aware model compression.

==> drafts/412_model_portability.tex <==
\section{experiments/accuracy-predictor-portability}
The accuracy-predictor used in \methodname~can be reused for search spaces different from the one it has been trained for, as long as the quality metrics for blocks in the new search space overlaps with those the predictor has been generated for. This is a major advantage for \methodname~since \textit{a)} the cost of generating the accuracy predictor can be amortized over different searches, and \textit{b)} it enables to extend an existing search space by including newer layers that today are appearing at a fast pace given the activities in deep-learning research field.

In this work we validate the portability of \methodname~accuracy predictor along two case studies: \textit{a)} for an \textit{extended search space} where a predictor trained for a given search space is validated on an augmented search space including additional type of layers, and \textbf{b)} quantization, where the predictor trained for full-precision blocks and networks search is validated for the quantized blocks and networks.

\textbf{Extended search space.} \textbf{TODO: take only validation data from the previously written section.}

\textbf{Quantized.} \textbf{TODO: take only validation data from the previously written section.}

The \methodname~approach can also be used for \textit{rapid search space design and exploration}. Using \methodname, a designer can quickly determine whether the search space should be extended or constrained for optimal performance.

 \input{figures_tex/figure_search_space_analysis}
%For example, the accuracy predictor generalizes to search-spaces with the same reference model but other macro-architectural variations such as ShiftNets~\cite{shiftnet} as replacement of depthwise-separable layers. 
Such extension is possible because the \methodname~accuracy predictor generalizes to previously unseen architectures, without having to extend the Architecture Library. 
Figure~\ref{fig:search_space_analysis}(left) shows this extrapolation works when extending to blocks based on ShiftNets~\cite{shiftnet}. Note how the trendline predicts the performance of full Pareto optimal ShiftNets even though the predictor is created without any ShiftNet data. Here, ShiftNets are our implementation, with learned shifts per group of 32 channels depthwise-separable replacement. These generalization capabilities are obtained because the predictor only uses BKD quality metrics as an input without requiring any structural information about the replacement block. 
%In our experiments, the accuracy predictor holds for the extended search space, as long as the distribution of the used quality metrics overlaps with the distribution of the quality metrics of the original search space. 
This feature is a major advantage of~\methodname~compared to OFA~\cite{ofa} and other methods where the predictor cannot automatically generalize to completely different layer-types, or to blocks of the same layer-type with parameters (expansion rate, kernel size, depth, ...) outside of the original search space.


%Figure~\ref{fig:search_space_analysis}(left) illustrates thisFor example, the baseline accuracy predictor for~\methodname, that does not include ShiftNets, can be used to predict the performance of architectures with such layer-types included. 
%To this end, the Block Library $B_{n,m}$ has to be extended through the BKD process (Section~\ref{sec:search_method}) to derive quality metrics for the new layer type, but no new targets are required and the predictor does not have to be retrained.
%All that is required to use the prior predictor for networks outside of the original search-space, is to go through the BKD (Section~\ref{sec:search_method}) process to extend the library of quality metrics and to initialize the weights of the added blocks for finetuning. 
%If $K$ replacement blocks are added to the extended search-space ($N \times K$ throughout the network), this only requires $N \times K$ epochs of additional BKD training. 

%In this case, it is always beneficial to use SE and Swish to maximimize accuracy for a given number of operations. Using ShiftNets appears to be never beneficial for $\#$ operations. 

This quick prototyping capability is also showcased for the \methodname~search space on a V100 GPU in Figure~\ref{fig:search_space_analysis}(right). We now use the original accuracy predictor to interpolate in the \methodname~search space, but estimate the impact of variations and constraints for rapid design space exploration~\cite{radosavovic2020designing}. In doing this, Fig.~\ref{fig:search_space_analysis} shows a diverse search space is crucial to achieve good performance on the V100 GPU. Especially the impact of adding SE-attention~\cite{squeeze_excite} optimally is very large, predicting a 15$\%$ speedup at 77$\%$ accuracy (line C vs D), or a 1$\%$ accuracy boost at 26ms (line E vs D). The full \methodname~space finds networks that are $30\%$ faster than a similar space with fewer choices in expansion ratios and with Squeeze-and-Excite in every block (line DONNA vs C). Every plotted line in Figure~\ref{fig:search_space_analysis} (right) is a predicted Pareto-optimal front for a variation of the search space. A baseline (A) considers SE and swish in every block and k $\in$ \{7\}, expand $\in$ \{3,4,6\} and depth $\in$ \{2,3,4\}. Other lines show results for search spaces built starting from (A), e.g. (B) considers k $\in$ \{5,7\}, (C) k $\in$ \{3,5,7\}, (D) removes SE and swish, (E) allows choosing optimal placement of SE and Swish, (F) adds a channel-width multiplier and full~\methodname~adds expand $\in$ \{2,3,4,6\} and depth $\in$ \{1,2,3,4\} and channel-scaling $\in$ \{0.5,1.0\}. 
%This approach quickly shows the impact of choices in the search space on real hardware, without requiring a novel predictor. 
%\methodname~hereby identifies Pareto-fronts for a partial or extended search space at a limited cost, especially where an accuracy predictor is already available.

==> figures_tex/figure_V100.tex <==
\begin{figure}
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{./figures/compare_V100_32.png}
  \caption{Nvidia V100, Batch Size 32, impact of search-space diversity}
  \label{fig:v1001}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{./figures/compare_v100_32_compare_searchspaces.png}
  \caption{Nvidia V100, Batch Size 32, impact of search-space diversity}
  \label{fig:v1002}
\end{subfigure}
\caption{plots of....}
\label{fig:fig}
\end{figure}


==> figures_tex/figure_cifar10_experiments.tex <==
\begin{figure*}[!h]
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=.90\linewidth]{./figures/cifar10_mbconvblock_acc.png}
  \label{fig:params}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=.90\linewidth]{./figures/cifar10_mbconvblockgroup32_acc.png}
  \label{fig:flops}
\end{subfigure}
\caption{Performance of accuracy predictors on different search spaces for MBConvBlock (left) and MBConvBlockGroup32 (right) mother networks.}
\label{fig:cifar10}
\end{figure*}

==> figures_tex/figure_flops_params.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{./figures/compare_PARAMS_32.png}
  \label{fig:params}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{./figures/compare_FLOPS_32.png}
  \label{fig:flops}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{./figures/compare_V100_32.png}
  \label{fig:gpu}
\end{subfigure}%
\caption{Trendlines and models found by \methodname~optimizing for the number of parameters (left), operations (mid) and inference time on an Nvidia V100 GPU (right).}
\label{fig:fig}
\end{figure*}


==> figures_tex/figure_flops_params_gpu.tex <==
\begin{figure*}[!t]
\centering
 \includegraphics[width=.99\linewidth]{./figures/4-pareto-fronts-magellan.pdf}
%\caption{Trendlines and models found by \methodname~optimizing for the number of parameters (left), a simulator targeting tensor compute units in a mobile SoC (mid left), inference time on an Nvidia V100 GPU (mid right) and a commercially available mobile device (right).}
\caption{The predicted Pareto-optimal front and models found by~\methodname~in the ~\methodname-, MobileNetV3-1.0x and MobileNetV3-1.2x search space. Results are shown targetting the number of operations (left), the number of parameters (mid left), latency on an Nvidia V100 GPU (mid right) and latency on a simulator targeting tensor compute units in a mobile SoC  (right). The trend line indicates predicted accuracy, whereas the dots are sampled from the predicted trend line and finetuned up to the level of from-scratch accuracy. Note that \methodname~finds architectures of the same quality as OFA~\cite{ofa} and Mnasnet~\cite{mnasnet} when comparing under similar training. On top of that, the \methodname~search space outperforms the MobileNetV3-style search spaces on-device. OFA* results are reproduced results using the framework in~\cite{ofa_repo}.}

\label{fig:trendlines_overview}
\end{figure*}


==> figures_tex/figure_flops_params_gpu_old.tex <==
\begin{figure*}[!t]
\centering
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{./figures/compare_PARAMS_32.png}
  \label{fig:params}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{./figures/compare_FLOPS_32.png}
  \label{fig:flops}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{./figures/compare_V100_32.png}
  \label{fig:gpu}
\end{subfigure}%
\caption{Trendlines and models found by \methodname~optimizing for the number of parameters (left), operations (mid) and inference time on an Nvidia V100 GPU (right).}
\label{fig:fig}
\end{figure*}


==> figures_tex/figure_kona.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=.8\linewidth]{./figures/compare_KONA_32.png}
\caption{Measurements on Snapdragon 865 mobile GPU. }
\label{fig:kona}
\end{figure}


==> figures_tex/figure_ranking_metrics_old.tex <==
\begin{figure}
\centering
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{./figures/linear_fit_pretty_ofa_best_L2TNorm.png}
  \caption{Predicted vs real accuracy of linear predictor.}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{./figures/ranking_ofa_best_L2TNorm.png}
  \caption{DNA~\cite{blockwise_nas} ranking vs ranking of linear model.}
  \label{fig:sfig2}
\end{subfigure}
\caption{Predictions and ranking, MobileNetV3 (1.2x).}
\label{fig:fig}
\end{figure}

==> figures_tex/supplementary_finetuning_speed.tex <==
\begin{figure}[t]
\centering
 \includegraphics[width=.99\linewidth]{./figures/finetuning-speed.pdf}
\caption{Speed at which BKD-initialized subsampled models can be finetuned for different search spaces. Models in ~\methodname, EfficientNet and ProxyLessNas (1.3$\times$) converge to the accuracy of 450-epoch from scratch training in less than 50 epochs using the BKD initialization point, a $9\times speedup$. Models in the MobileNetV3 search space converge in about 30 epochs, a $15\times$ speedup. If the supernet from OFA~\cite{ofa_repo,ofa} is used as a reference model and teacher model in the \methodname pipeline for MobileNetV3 (1.2$\times$), from-scratch 450 epoch accuracy is even achieved in less than 15 epochs, a $30\times$ speed up.}
\label{fig:supplementary/finetuning-speed}
\end{figure}

==> figures_tex/supplementary_flops_params_gpu.tex <==
\begin{figure*}[t]
\centering
 \includegraphics[width=.99\linewidth]{./figures/4-pareto-fronts-all.pdf}
\caption{Trendlines and models found by \methodname~optimizing for the number of parameters (left), the number of operations (mid left), inference time on an Nvidia V100 GPU (mid right) and a commercially available Samsung S20 smartphone GPU (right). Best viewed in color.}
\label{fig:supplementary/search-space-overview}
\end{figure*}

==> supplementary_material/01_ablation.tex <==
\section{Ablation Study} \label{sec:ablation}
\subsection{Block Transplantation and Blockwise Knowledge Distillation}
Discuss impact of learning schedule (learning rate, optimizer, number of steps, loss function).

\subsection{Training schemes for Blockwise Knowledge Distillation}
Discuss impact of learning schedule (learning rate, optimizer, number of steps, loss function).

\subsection{Choice of Mother Network}

\input{figures_tex/figure_cifar10_experiments}

One of the most important choices to make before doing the whole QUARTS procedure is choosing a mother network. Since it will be used at every step of the procedure, choosing a wrong one might result in multiple issues: (1) blocks trained with knowledge distillation might not reach satisfying accuracy; (2) built accuracy predictor might give a wrong estimate for the selected search space; (3) due to knowledge distillation procedure in the finetuning, resulting models can have lower accuracy compared to using a better teacher.

The main assumption being used throughout the paper is that the best teacher is the largest one. This is in line with previous works \cite{yang2018knowledge,lan2018knowledge,yim2017agift}. However, another line of research \cite{cho2019efficacy} has shown that the biggest teachers might hinder the performance of students if those can't reach the same capacity as the teacher. We have not observed that in any of our experiments and we hypothesize that it is due to the blockwise training procedure which leads to easier optimization. Since we are trying to approximate per-block function it ends up being easier than approximating full model. 

To confirm our hypothesis even further, we conduct a set of experiments where we use two different mother networks as teachers - a larger one (MBConvBlockGroup32-based) and a smaller one (MBConvBlock-based). We then use those to build two accuracy models - one per teacher and assess accuracies of models consisting fully of  blocks and MBConvGroup32 blocks. As you can see in \ref{fig:cifar10}, using larger model allows for a good estimate for both MBConv and MBConvGroup32 models. However, when using smaller model, MBConvGroup32 models end up being highly underestimated since smaller teacher prevents models from learning further during blockwise kd training.

This confirms that when training on a new search space, the largest model in this search space should be used as a teacher.

==> tables/table_ofa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\iffalse
\begin{table*}[h]
\caption{\label{tab:ofa}hello }
\centering
\bgroup
\def\arraystretch{0.9}%
\begin{tabular}{l|c|c|c|c|c}
\multirow{2}{*}{Network} & ImageNet 224 & ImageNet FT & ImageNet Scratch & EffDet-D0 512 & MSCOCO 512 \\
& $\#$ operations & val top-1 $[\%]$ & val top-1 $[\%]$ & $\#$ operations & val mAP \\ \hline
OFA-FLOPS-224-A & 374 &  - & 77.26 & 2474 & 33.3 \\
OFA-FLOPS-224-B & 426 &  - & 77.64 & 2745 & 33.7 \\
OFA-FLOPS-224-C & 662 &  - & 78.66 & 3975 & 34.6 \\
OFA-FLOPS-A & 405 &  79.1@75 & 77.72 & 2632 & 33.9 \\
OFA-FLOPS-B & 618 &  80.0@75 & 79.09 & 3302 & 34.7 \\ \hline
DONNA-OFA-224-A & 406 & 77.3@50 & - & 2641 & 33.1 \\
DONNA-OFA-224-B & 501 & 77.9@50 & - & 3131 & 34.1 \\
DONNA-OFA-224-C & 599 & 78.3@50 & - & 3646 & 34.7 \\
\end{tabular}
\egroup
\end{table*}
\fi

\iffalse
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{\label{tab:ofa} \methodname~performs similar or better than OFA \cite{ofa} on MS-COCO object detection~\cite{coco} using the same MobileNetV3 ($1.2\times$) search-space as backbones in an EfficientDet-D0~\cite{efficientdet} setup. All networks are optimized minimizing the number of operations on ImageNet for a $224\times224$ input size. $^*$ published network\cite{ofa_repo}, $^\dagger$ our search using~\cite{ofa,ofa_repo} with input size fixed to $224\times224$.}
\centering
\bgroup
\def\arraystretch{1.0}%
\begin{tabular}{l|c|c}
\multirow{2}{*}{Network}  & EffDet-D0 & COCO \\
& operations [GOp] & Val mAP \\ \hline
OFA-A$^*$ & 2.6 & 33.9 \\
OFA-A$^\dagger$  & 2.5 & 33.3 \\
DONNA-A & 2.6 & 33.1 \\ \hline
OFA-B$^\dagger$  & 2.7 & 33.7 \\
DONNA-B & 3.1 & 34.1 \\ \hline
OFA-C$^\dagger$ & 4.0 & 34.6 \\
DONNA-C & \underline{\textbf{3.6}} & \underline{\textbf{34.7}} \\
\end{tabular}
\egroup
\end{table}
\fi

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[b]
\caption{\label{tab:ofa} \methodname~backbones perform similarly or better than OFA \cite{ofa} coming from the same MobileNetV3 ($1.2\times$) search space when transferred to object detection. All networks here replace the default backbone of  EfficientDet-D0~\cite{efficientdet}. All networks are optimized to minimize the number of operations on ImageNet for a $224\times224$ input size. Weights for OFA-A are from \cite{ofa_repo}. Backbones with $^\dagger$ are from our reproduction of OFA \cite{ofa,ofa_repo}. Models without @ are trained from scratch. \blueText{PN: I suggest we remove the table or move to Supp Mat. I've expanded the main text to make it more precise, and together with the plot, it should be sufficient to get our main points across.}}
\centering
\bgroup
\def\arraystretch{0.85}%
\begin{tabular}{l|c|c|c}
\multirow{2}{*}{Backbone} & ImageNet  & EffDet-D0 & COCO \\
& Val Top-1 & Ops [B] & Val mAP \\ \hline
OFA-A$^*$ & 79.1@75 & 2.6 & 34.1 \\
OFA224-A$^\dagger$ & 77.26  & 2.5 & 33.3 \\
DONNA-A & 77.3@50 & 2.6 & 33.1 \\ \hline
OFA224-B$^\dagger$ & 77.64  & 2.7 & 33.7 \\
DONNA-B & 77.95@50 & 3.1 & 34.1 \\ \hline
OFA224-C$^\dagger$ & 78.66 & 4.0 & 34.6 \\
DONNA-C & 78.38@50 & \underline{\textbf{3.6}} & \underline{\textbf{34.7}} \\
\end{tabular}
\egroup
\end{table}

==> tables/table_search_space.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[th]
\caption{\label{tab:search_space} Comparing the OFA search-space versus the \methodname~search-space, for every cell in Figure~\ref{fig:bkd_overview}. In \methodname, only the size of the intermediate feature maps between cells (denoted by $C_{in}$,$C_{out}$,$S=Stride$) needs to be fixed. }
\centering
\begin{tabular}{|c||c|c|c|c|c|c|c|}
\hline
Reference & $C_{in}$/$C_{out}$/$S$ & kernel - expand - depth & Layer & Attention & Activation & Granularity & Cost \\
\hline
OFA~\cite{ofa} & fixed & 3,5,7 - 3,4,6 - 2,3,4 & fixed & fixed & fixed & per layer & 1 \\
\methodname & fixed & 3,5,7 - 2,3,4,6 - 1,2,3,4 & DWS, G & SE/no-SE & ReLU/Swish & per block & 1 \\
MNASNet~\cite{mnasnet} & any & 3,5,7 - 2,3,4,6 - 1,2,3,4 & DWS & SE/no-SE & ReLU/Swish & per layer & 40 \\
\hline
\end{tabular}
\end{table*}

==> tables/table_search_space_full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{\label{tab:search_space}Your caption.}
\centering
\bgroup
\def\arraystretch{1.0}%
\begin{tabular}{|c||cccc|ccccccc|}
\hline
\multirow{2}{*}{Cell Index} & \multicolumn{4}{c|}{MobileNetV3 1.2x / ProxyLessNas 1.3x}& \multicolumn{6}{c|}{Quarts} \\

& SE/NL/$c$& r & k & e & SE & NL & $c$ & r & k & e    \\ 
\hline
0  & fixed & 2,3,4 & 3,5,7 & 3,4,6 & Y,N & S,R & 16,32 & 1,2,3,4 & 3,5,7 & 2,3,4,6 \\
1  & fixed & 2,3,4 & 3,5,7 & 3,4,6 & Y,N & S,R & 16,32 & 1,2,3,4 & 3,5,7 & 2,3,4,6 \\
2  & fixed & 2,3,4 & 3,5,7 & 3,4,6 & Y,N & S,R & 16,32 & 1,2,3,4 & 3,5,7 & 2,3,4,6 \\
3  & fixed & 2,3,4 & 3,5,7 & 3,4,6 & Y,N & S,R & 16,32 & 1,2,3,4 & 3,5,7 & 2,3,4,6 \\
4  & fixed & 2,3,4 & 3,5,7 & 3,4,6 & Y,N & S,R & 16,32 & 1,2,3,4 & 3,5,7 & 2,3,4,6 \\
\hline
\end{tabular}
\egroup
\end{table*}
